Enhancing Text Generation with Cooperative Training

Recently, there has been a surge in the use of generated data to enhance the performance of downstream models, largely due to the advancements in pre-trained language models. However, most prevailing methods trained generative and discriminative models in isolation, which left them unable to adapt to changes in each other. These approaches lead to generative models that are prone to deviating from the true data distribution and providing limited benefits to discriminative models. While some works have proposed jointly training generative and discriminative language models, their methods remain challenging due to the non-differentiable nature of discrete data. To overcome these issues, we introduce a \textit{self-consistent learning} framework in the text field that involves training a discriminator and generator cooperatively in a closed-loop manner until a scoring consensus is reached. By learning directly from selected samples, our framework are able to mitigate training instabilities such as mode collapse and non-convergence. Extensive experiments on four downstream benchmarks, including AFQMC, CHIP-STS, QQP, and MRPC, demonstrate the efficacy of the proposed framework.

==> Table/datasets.tex <==
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt} % 列间距
\caption{Statistics of Experimental Datasets}
\label{dataset}
\begin{tabular}{cccccc}
\toprule
 &  & AFQMC & CHIP-STS & QQP-ZH & MRPC \\ \midrule
\multirow{2}{*}{Zero-Shot} & \begin{tabular}[c]{@{}c@{}}domain-related\\ corpus\end{tabular} & 68668 & 32000 & 10800 & 8,152 \\
 & test dataset & 4316 & 4000 & 3600 & 1725 \\ \midrule
\multirow{2}{*}{Fine-Tune} & training dataset & 34334 & 16000 & 5400 & 4076 \\ 
 & test dataset & 4316 & 4000 & 3600 & 1725 \\ \bottomrule
\end{tabular}
\end{table}

==> Table/kl.tex <==
\begin{table}
\small
\centering
\setlength\tabcolsep{8pt} % 列间距
\caption{The KL divergence in the First and Last rounds of Zero-Shot.}
\label{consistent}
\sc
\begin{tabular}{l|cc}
\toprule
 & \begin{tabular}[l]{@{}r@{}}KL Divergence\\ \textit{-first round}\end{tabular} & \begin{tabular}[l]{@{}r@{}}KL Divergence\\ \textit{-last round}\end{tabular} \\ \midrule
AFQMC & 0.29 & 0.26 \\
CHIP-STS & 0.16 & 0.08 \\
QQP-ZH & 0.18 & 0.06 \\
MRPC &0.22 & 0.02 \\ \bottomrule
\end{tabular}
\end{table}

==> Table/para_finetune.tex <==
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt} % 列间距
\caption{Parameter Settings of Fine-Tune.}
\label{fine-tune-parm}
\begin{tabular}{l|cccc}
\toprule
 & AFQMC & CHIP-STS & QQP-ZH & MRPC \\\midrule
\begin{tabular}[l]{@{}r@{}}Max Threshold\\ \textit{-negative}\end{tabular} & 0.98 & 0.98 & 0.84 & 0.8 \\ 
\begin{tabular}[l]{@{}r@{}}Min Threshold\\ \textit{-negative}\end{tabular} & 0.9 & 0.7 & 0.6 & 0.6 \\ 
\begin{tabular}[l]{@{}r@{}}Max Threshold\\ \textit{-positive}\end{tabular} & 0.98 & 0.98 & 0.98 & 0.8 \\
\begin{tabular}[l]{@{}r@{}}Min Threshold\\ \textit{-positive}\end{tabular} & 0.9 & 0.7 & 0.9 & 0.6 \\ 
\begin{tabular}[l]{@{}r@{}}Max Threshold\\ \textit{-generator}\end{tabular} & 0.98 & 0.98 & 0.98 & 0.8 \\ 
\begin{tabular}[l]{@{}r@{}}Min Threshold\\ \textit{-generator}\end{tabular} & 0.9 & 0.7 & 0.9 & 0.6 \\ 
Threshold Increase & 0.07 & 0.07 & 0.07 & 0.2 \\
Sentence Num & 6000 & 6000 & 3000 & 3000 \\
Learning Rate & \multicolumn{4}{c}{5e-6} \\
Warm Up Steps & \multicolumn{4}{c}{40} \\
Early Stopping & \multicolumn{4}{c}{1} \\
\begin{tabular}[c]{@{}r@{}}$\mathcal{G}$ Batch Size\\\textit{ -training}\end{tabular} & \multicolumn{3}{c}{2(concat 30 samples)} & 24 \\
\begin{tabular}[l]{@{}r@{}}$\mathcal{G}$ Batch Size\\\textit{ -predicting}\end{tabular} & \multicolumn{3}{c}{512} & 100 \\
\begin{tabular}[l]{@{}r@{}}$\mathcal{D}$ Batch Size\\ \textit{-training}\end{tabular} & 32 & 64 & 32 & 32 \\ 
\begin{tabular}[l]{@{}r@{}}$\mathcal{D}$ Batch Size\\ \textit{-predicting}\end{tabular} & 256 & 384 & 256 & 96 \\ \bottomrule
\end{tabular}
\end{table}

==> Table/para_zeroshot.tex <==
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt} % 列间距
\caption{Parameter Settings of Zero-Shot.}
\label{zero-shot-parm}
\begin{tabular}{l|cccc}
\toprule
 & AFQMC & CHIP-STS & QQP-ZH & MRPC \\ \midrule
\begin{tabular}[l]{@{}r@{}}Max Threshold\\ \textit{-negative}\end{tabular} & 0.8 & 0.9 & 0.95 & 0.95 \\ 
\begin{tabular}[l]{@{}r@{}}Min Threshold\\ \textit{-negative}\end{tabular} & 0.6 & 0.7 & 0.8 & 0.8 \\ 
\begin{tabular}[l]{@{}r@{}}Max Threshold\\ \textit{-positive}\end{tabular} & 0.8 & 0.9 & 0.95 & 0.95 \\ 
\begin{tabular}[l]{@{}r@{}}Min Threshold\\ \textit{-positive}\end{tabular} & 0.6 & 0.7 & 0.8 & 0.8 \\ 
\begin{tabular}[l]{@{}r@{}}Max Threshold\\ \textit{-generator}\end{tabular} & 0.6 & 0.9 & 0.95 & 0.95 \\ 
\begin{tabular}[l]{@{}r@{}}Min Threshold\\ \textit{-generator}\end{tabular} & 0.6 & 0.7 & 0.8 & 0.8 \\ 
Threshold Increase & 0.07 & 0.1 & 0.05 & 0.05 \\
Sentence Num & 6000 & 6000 & 3000 & 4000 \\ 
Learning Rate & \multicolumn{4}{c}{2e-5} \\ 
Warm Up Steps & \multicolumn{4}{c}{40} \\ 
Early Stopping & \multicolumn{4}{c}{1} \\ 
\begin{tabular}[l]{@{}r@{}}$\mathcal{G}$ Batch Size\\ \textit{-training}\end{tabular} & \multicolumn{3}{c}{2(concat 30 samples)} & 24 \\ 
\begin{tabular}[l]{@{}r@{}}$\mathcal{G}$ Batch Size\\ \textit{-predicting}\end{tabular} & \multicolumn{3}{c}{512} & 100 \\ 
\begin{tabular}[l]{@{}r@{}}$\mathcal{D}$ Batch Size\\ \textit{-training}\end{tabular} & \multicolumn{3}{c}{64} & 32 \\ 
\begin{tabular}[l]{@{}r@{}}$\mathcal{D}$ Batch Size\\ \textit{-predicting}\end{tabular} & \multicolumn{3}{c}{384} & 96 \\ \bottomrule
\end{tabular}
\end{table}
